Real-Time VPN Traffic over ETSI GS QKD 014 Key Delivery with a LuxQuanta NOVA QKD Platform

This report presents a prototype VPN that uses QKD-derived keys delivered through the ETSI GS QKD 014 API. The VPN encrypts IP traffic with AES-256-GCM, transports ETSI key identifiers in-band, and retrieves matching keys from local KMEs. After validation with a controlled KME simulator, the system was tested on two Jetson Xavier NX devices connected to a LuxQuanta NOVA QKD platform. The experiment successfully transmitted bidirectional real-time audio and video traffic through the VPN for eight continuous hours, demonstrating the feasibility of integrating classical VPN applications with QKD infrastructure through a standardized key-delivery interface.

==> tex/annex/operacoes_complexas.tex <==
Para contabilizar as operações básicas (soma e multiplicação) necessárias para realizar operações entre dois números complexos, é necessário primeiramente analisar cada operação separadamente.

Considerando dois números complexos na forma:

$a = a_r + a_i i$

$b = b_r + b_i i$

Onde $a_r$, $a_i$, $b_r$ e $b_i$ são números reais.

\section{Soma de Números Complexos}

A soma de dois números complexos é dada por:

$(a_r + a_i i) + (b_r + b_i i) = (a_r + b_r) + (a_i + b_i)i$

Operações necessárias:

\begin{itemize}
    \item 2 somas reais (uma para a parte real e outra para a parte imaginária)
    \item 0 multiplicações reais
\end{itemize}

% TODO: verificar
\section{Multiplicação de Números Complexos}

A multiplicação de dois números complexos é dada por:

$(a_r + a_i i) \times (b_r + b_i i) = (a_r \times b_r - a_i \times b_i) + (a_r \times b_i + a_i \times b_r)i$

Operações necessárias:

\begin{itemize}
    \item 2 somas/subtrações reais (uma subtração para a parte real e uma soma para a parte imaginária)
    \item 4 multiplicações reais ($a_r \times b_r$, $a_i \times b_i$, $a_r \times b_i$, $a_i \times b_r$)
\end{itemize}

% TODO: verificar
\section{Divisão de Números Complexos}

A divisão de dois números complexos pode ser calculada como:

$\frac{a_r + a_i i}{b_r + b_i i} = \frac{(a_r + a_i i)(b_r - b_i i)}{(b_r + b_i i)(b_r - b_i i)} = \frac{(a_r b_r + a_i b_i) + (a_i b_r - a_r b_i)i}{b_r^2 + b_i^2}$

Operações necessárias:

\begin{itemize}
    \item 5 somas/subtrações reais (2 para o numerador e 1 para o denominador, mais 2 para a normalização final)
    \item 6 multiplicações reais (4 para o numerador, 2 para o denominador)
    \item 2 divisões reais (que podem ser decompostas em multiplicações pelo inverso)
\end{itemize}

% TODO: verificar
\section{Raiz Quadrada de um Número Complexo}

Para calcular a raiz quadrada de um número complexo $a = a_r + a_i i$, podemos usar a forma polar:

\begin{enumerate}
    \item Converter para forma polar: $a = |a|e^{i\theta}$ onde $|a| = \sqrt{a_r^2 + a_i^2}$ e $\theta = \arctan(a_i/a_r)$
    \item Calcular a raiz: $\sqrt{a} = \sqrt{|a|}e^{i\theta/2}$
    \item Converter de volta para forma retangular: $\sqrt{a} = \sqrt{|a|}\cos(\theta/2) + i\sqrt{|a|}\sin(\theta/2)$
\end{enumerate}

Operações necessárias:

\begin{itemize}
    \item Aproximadamente 8 somas/subtrações reais
    \item Aproximadamente 8 multiplicações reais
    \item 2 operações de raiz quadrada real
    \item 2 operações trigonométricas (seno e cosseno)
    \item 1 operação de arcotangente
\end{itemize}

% As operações trigonométricas e a raiz quadrada real podem ser decompostas em séries de operações básicas, mas a contagem exata dependerá do algoritmo específico utilizado para implementá-las.

% Em resumo, a complexidade computacional em termos de operações básicas aumenta significativamente à medida que passamos da soma (mais simples) para a raiz quadrada (mais complexa).

==> tex/annex/operacoes_equacoes.tex <==
As operações elementares para cada bloco do sistema foram estimadas a partir dos algoritmos implementados no \textit{framework CV-QKD-ModSim}. A partir da análise individual de cada algoritmo foram definidas equações parametrizáveis aproximadas para contabilizar somas/subtrações, multiplicações, divisões, raiz quadrada, leitura e escrita de dados.

Na Tabela \ref{tab:parametros} estão descritos os parâmetros que influenciam na quantidade de operações realizadas, juntamente com os símbolos que serão utilizados na descrição das equações.

\begin{table}[htpb]
\renewcommand{\arraystretch}{1.2}
\centering
\caption{Parâmetros e seus respectivos símbolos}
\label{tab:parametros}
\begin{tabular}{ll}\toprule
\textbf{Parâmetro} & \textbf{Símbolo} \\ \midrule
Total de bits transmitidos& $N_{bits}$  \\
Total de símbolos no transmissor& $Tx_{\text{symbols}}$  \\
Total de amostras no transmissor& $Tx_{\text{samples}}$  \\
Total de símbolos no receptor& $Rx_{\text{symbols}}$  \\
Total de amostras no receptor& $Rx_{\text{samples}}$  \\
Tamanho da constelação& $M$                   \\
Quantidade de modos                 & $N_{\text{modes}}$    \\
Comprimento do conformador de pulso & $N_{\text{RRC}}$      \\
Valor de compensação& $N_{\text{comp}}$  \\
Comprimento do equalizador adaptativo  & $L_{\text{eq}}$    \\
Nº de fases de teste para algoritmo BPS   & $N_{\phi}$      \\
Tamanho da janela para algoritmo BPS/Viterbi& $N_{\text{window}}$ 
\\ \bottomrule\end{tabular}
\end{table}

As Tabelas \ref{tab:equacoes} e \ref{tab:equacoesRW} descrevem as equações aproximadas para cada operação considerando números complexos, exceto para o bloco Descasador de Distribuição, onde são contabilizadas as operações com números reais (operações simples). Sendo a primeira para operações matemáticas e a segunda para os processos de leitura e escrita.

% \begin{table}[htpb]
% \renewcommand{\arraystretch}{1.5}
% \centering
% \caption{Parâmetros e seus respectivos símbolos}
% \label{tab:equacoes}
% \begin{adjustbox}{max width=\textwidth}
% \begin{tabular}{m{10em} m{15em} m{20em} m{8em} l}\toprule
% \textbf{Bloco} & \textbf{Soma} & \textbf{Multiplicação} & \textbf{Divisão} & \textbf{Raiz Quadrada} \\ \midrule
% \textbf{Transmissor} &&&&\\
% Casador de Distribuição & $17 \cdot M + 4 \cdot Tx_{\text{symbols}} + 201$ &
% $2 \cdot Tx_{\text{symbols}}$ &
% $5 \cdot M + 102$& - \\
% Modulação Digital &&&& \\
% \textit{Upsampling} &&&& \\
% Formatador de pulso RRC & $Tx_{\text{samples}} \cdot N_{\text{RRC}} - 1$&$Tx_{\text{samples}} \cdot N_{\text{RRC}}$&&\\
% \textbf{Receptor} &&&&\\ 
% Filtragem Casada RRC &$Rx_{\text{samples}} \cdot N_{\text{RRC}}$&$Rx_{\text{samples}} \cdot (N_{\text{RRC}} - 1)$&--& --\\
% Sincronização de Símbolo e Decimação &&&& \\
% Compensação da Dispersão \\ Cromática &$6 \cdot N_{\text{comp}} \cdot \log_2(N_{\text{comp}})$&$4 \cdot N_{\text{comp}} \cdot \log_2(N_{\text{comp}})$&& \\
% Estimativa de Offset de Frequência&$3 \cdot N_{\text{comp}} + N_{\text{comp}} \cdot \log_2(N_{\text{comp}})$&$12 \cdot N_{\text{comp}} + N_{\text{comp}} \cdot \log_2(N_{\text{comp}}) + 3$&& \\
% Equalização Adaptativa &$N_{\text{comp}}^2 \cdot N_{\text{modes}}^2 + (N_{\text{comp}}^2 + 2) \cdot N_{\text{modes}} + 2 \times (N_{\text{comp}} - 1) + N_{\text{comp}} \cdot N_{\text{RRC}} \cdot (N_{\text{modes}} - 1 + N_{\text{modes}}^2) + N_{\text{comp}} \cdot N_{\text{modes}}$&$N_{\text{comp}}^2 \cdot N_{\text{modes}}^2 + N_{\text{comp}}^2 \cdot N_{\text{modes}} + N_{\text{comp}} + N_{\text{comp}} \cdot N_{\text{RRC}} \cdot (N_{\text{modes}} + N_{\text{modes}}^2) + N_{\text{comp}} \cdot N_{\text{modes}}$&$2 \cdot N_{\text{comp}}$& $2$\\
% Recuperação da Fase de Portadora &$N_{\text{modes}} \left( \log(N_{\text{comp}}) + 2 \times \frac{N_{\text{comp}} - 1}{N_{\text{comp}}} + B \times (M + 2 \times N) \right)$&$N_{\text{modes}} \left(4 + \log(N_{\text{comp}}) + B \times (1 + M)\right)$&& \\
% Correção de Rotações Residuais &$10 \times (Tx_{\text{symbols}} - 1) + 4 \times Tx_{\text{symbols}}$&$10 \times Tx_{\text{symbols}}$&$4 + 10 \times Tx_{\text{symbols}}$& $10$\\
% Descasador de Distribuição &$ \left( N_{\text{mod}} \times (30 \times M^{2} + 48 \times M + 10) + 4 \times M + 1 \right) + \left( N_{\text{modes}} \times M \times N_{\text{mod}} \right) $&$ N_{\text{mod}} \times (12 \times M + 3) + 2 \times N_{\text{modes}} \times M \times N_{\text{mod}} $&$ N_{\text{mod}} \times (3 \times M^{2} + 12 \times M) + M $& $ N_{\text{modes}} \times M \times N_{\text{mod}} $\\
% \bottomrule
% \end{tabular}
% \end{adjustbox}
% \end{table}

\begin{table}[htpb]
\renewcommand{\arraystretch}{1.5}
\centering
\caption{Equações para a estimativa de operações matemáticas com números complexos}
\label{tab:equacoes}
\scriptsize % Reduz o tamanho da fonte
\begin{adjustbox}{max width=\textwidth}
\begin{threeparttable}[b]
\begin{tabular}{p{10em} p{15em} p{15em} p{10em} p{7em}}
\toprule
\textbf{Bloco} & \textbf{Soma/Subtração} & \textbf{Multiplicação} & \textbf{Divisão} & \textbf{Raiz Quadrada} \\ 
\midrule
\textbf{Transmissor} &&&&\\ 
Casador de Distribuição & $17 \cdot M + 4 \cdot Tx_{\text{symbols}} + 201$ & $2 \cdot Tx_{\text{symbols}}$ & $5 \cdot M + 102$ & --\\
Modulação Digital &--&--&--& --\\
\textit{Upsampling} &--&--&--& --\\
Formatador de pulso RRC & $Tx_{\text{samples}} \cdot N_{\text{RRC}} - 1$ & $Tx_{\text{samples}} \cdot N_{\text{RRC}}$ &--& --\\
\textbf{Receptor} &&&& \\
Filtragem Casada RRC & $Rx_{\text{samples}} \cdot N_{\text{RRC}}$ & $Rx_{\text{samples}} \cdot (N_{\text{RRC}} - 1)$ & --& --\\
Sincronização de Símbolo e Decimação &--&--&--& --\\
Compensação da Dispersão Cromática & $6 \cdot N_{\text{comp}} \cdot \log_2(N_{\text{comp}})$ & $4 \cdot N_{\text{comp}} \cdot \log_2(N_{\text{comp}})$ &--& --\\
Estimativa de Offset de Frequência & $3 \cdot N_{\text{comp}} + N_{\text{comp}} \cdot \log_2(N_{\text{comp}})$ & $12 \cdot N_{\text{comp}} + N_{\text{comp}} \cdot \log_2(N_{\text{comp}}) + 3$ &--& --\\
Equalização Adaptativa & $N_{\text{comp}}^2 \cdot N_{\text{modes}}^2 + (N_{\text{comp}}^2 + 2) \cdot N_{\text{modes}} + 2(N_{\text{comp}} - 1) + N_{\text{comp}} \cdot N_{\text{RRC}} \cdot (N_{\text{modes}} - 1 + N_{\text{modes}}^2) + N_{\text{comp}} \cdot N_{\text{modes}}$ & $N_{\text{comp}}^2 \cdot N_{\text{modes}}^2 + N_{\text{comp}}^2 \cdot N_{\text{modes}} + N_{\text{comp}} + N_{\text{comp}} \cdot N_{\text{RRC}} \cdot (N_{\text{modes}} + N_{\text{modes}}^2) + N_{\text{comp}} \cdot N_{\text{modes}}$ & $2 \cdot N_{\text{comp}}$ & $2$ \\
Recuperação da Fase de Portadora & $N_{\text{modes}} (\log(N_{\text{comp}}) + 2 \cdot \frac{N_{\text{comp}} - 1}{N_{\text{comp}}} + B \cdot (M + 2N))$ & $N_{\text{modes}} (4 + \log(N_{\text{comp}}) + B \cdot (1 + M))$ &--& --\\
Correção de Rotações Residuais & $10 \cdot (Tx_{\text{symbols}} - 1) + 4 \cdot Tx_{\text{symbols}}$ & $10 \cdot Tx_{\text{symbols}}$ & $4 + 10 \cdot Tx_{\text{symbols}}$ & $10$ \\
Descasador de Distribuição \tnote{1} & $(N_{\text{mod}} \cdot (30 M^{2} + 48 M + 10) + 4 M + 1) + (N_{\text{modes}} \cdot M \cdot N_{\text{mod}})$ & $N_{\text{mod}} \cdot (12 M + 3) + 2 N_{\text{modes}} M N_{\text{mod}}$ & $N_{\text{mod}} \cdot (3 M^{2} + 12 M) + M$ & $N_{\text{modes}} \cdot M \cdot N_{\text{mod}}$ \\
\bottomrule
\end{tabular}
\begin{tablenotes}
\item[1] Equação aproximada para operações com valores reais.
\end{tablenotes}
\end{threeparttable}
\end{adjustbox}
\end{table}


\begin{table}[htpb]
\renewcommand{\arraystretch}{1.2}
\centering
\caption{Equações para a estimativa de operações de leitura e escrita em memória}
\label{tab:equacoesRW}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lll}\toprule
\textbf{Bloco} & \textbf{Leitura} & \textbf{Escrita} \\ \midrule
\textbf{Transmissor} &&\\
Casador de Distribuição & $4 \cdot Tx_{\text{symbols}} + 11 \cdot M$& $2 \cdot Tx_{\text{symbols}} + Tx_{\text{symbols}} \cdot M + 2 \cdot M$ \\ 
Modulação Digital & $N_{\text{bits}} + M$ & $Tx_{\text{symbols}}$ \\ 
\textit{Upsampling} &$Tx_{\text{symbols}}$&$Tx_{\text{samples}}$ \\ 
Formatador de pulso RRC & $Tx_{\text{samples}} + N_{\text{RRC}}$& $Tx_{\text{samples}}$\\ 
\textbf{Receptor} &&\\ 
Filtragem Casada RRC &$N_{\text{RRC}} + Rx_{\text{samples}}$& $Rx_{\text{samples}}$\\
Sincronização de Símbolo e Decimação &$Rx_{\text{samples}}$& $N_{\text{comp}}$\\
Compensação da Dispersão Cromática &$2 \cdot N_{\text{comp}}$& $N_{\text{comp}}$\\
Estimativa de Offset de Frequência &$N_{\text{comp}}$& $N_{\text{comp}}$\\
Equalização Adaptativa &$N_{\text{comp}} + Tx_{\text{symbols}}$& $Tx_{\text{symbols}}$\\
Recuperação da Fase de Portadora &$Tx_{\text{symbols}} + M$& $Tx_{\text{symbols}}$\\
Correção de Rotações Residuais & $2 \times Tx_{\text{symbols}}$& $Tx_{\text{symbols}}$\\
Descasador de Distribuição &$ N_{\text{mod}} + 5 \times M $& $ 2 \times N_{\text{mod}} $\\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}



==> tex/background.tex <==
\chapter{Fundamentos}
\label{chapter:background}

% Tem que arrumar as referências

A criptografia desempenha um papel importante há milhares de anos e continua mantendo a sua importância no mundo moderno, sendo essencial para o funcionamento seguro da nova geração tecnológica. Atualmente existem dois tipos de criptografia de chave: a criptografia de chave privada, também chamada de criptografia simétrica, e a criptografia de chave pública, também conhecida como criptografia assimétrica \cite{peterson2007computer}.   

Na criptografia simétrica, o remetente e o destinatário compartilham uma mesma chave secreta, utilizada tanto para encriptar quanto para decriptar. Caso essa chave seja vazada para alguém que não deva ter acesso, a troca de mensagens estará comprometida. Um problema nessa abordagem é a necessidade de distribuir essa chave entre ambas as partes antes de iniciar a troca de mensagens.  

A criptografia assimétrica utiliza um par de chaves: a chave pública, que pode ser divulgada, e a chave privada, que deverá se manter em sigilo. Em geral, as duas abordagens são combinadas: a criptografia assimétrica para garantir a autenticidade e, assim, realizar a troca de uma chave secreta entre duas partes. Com a chave secreta definida, as partes passam a se comunicar por meio de criptografia simétrica. Sem algoritmos de criptografia assimétrica, seria necessário que as chaves fossem pré-compartilhadas entre as partes de outra maneira, por exemplo, configuradas fisicamente por um administrador. Essa abordagem é conhecida como \gls{PSK} \cite{cano2024line}.

Com o enfraquecimento dos algoritmos de criptografia assimétrica baseados no problema de fatoração causado pelo advento das tecnologias quânticas, novos algoritmos estão sendo propostos como os algoritmos ML-KEM, usado para estabelecer chaves criptográficas seguras e ML-DSA para assinaturas digitais, ambos padronizados pelo Instituto Nacional de Padrões e Tecnologia (NIST). Esses algoritmos são chamados de \gls{PQC}, e se baseiam em problemas matemáticos projetados para serem mais resistentes ao poder computacional quântico. Enquanto a PQC foca em criar uma matemática mais complexa para substituir os algoritmos dentro da infraestrutura clássica, por outro lado, a QKD usa utiliza as próprias leis da mecânica quântica para entregar chaves de forma incondicionalmente segura, extinguindo de vez a necessidade da criptografia assimétrica para essa função.

\section{Protocolos QKD}

O paradigma do que é um protocolo de distribuição quântica de chaves pode ser entendido a partir de uma perspectiva da teoria da informação, como um conjunto de regras e convenções que estabelecem como os dados são preparados, transmitidos, recebidos e acessados entre dispositivos~\cite{tacla}. Se reduzirmos um cenário de comunicação à sua estrutura mais simples, podemos modelar duas partes espacialmente separadas (comumente chamadas de Alice e Bob) que querem se comunicar por algum meio, usando mensagens cifradas. A ideia central é que apenas Alice e Bob tenham conhecimento do conteúdo de suas mensagens e que nenhuma terceira parte (comumente chamada Eva) possa acessar a chave secreta.  

Os sistemas de criptografia clássicos usados atualmente, como o modelo RSA, são baseados no compartilhamento de chaves criptográficas (sequências aleatórias de números binários) públicas entre Alice e Bob e sua segurança é garantida exclusivamente pela dificuldade computacional envolvida na tentativa de decifragem dessa chave por Eva. Avanços tecnológicos, como o desenvolvimento de computadores quânticos, representam um risco para a segurança desses protocolos. O algoritmo de ~\cite{shor} prova que atualmente um computador quântico se tornou capaz de resolver problemas matemáticos complexos como a fatoração de grandes números, a base da RSA, destruindo assim a sua segurança em um tempo totalmente hábil em comparação a computadores clássicos. 

Em contrapartida, nos protocolos de criptografia quântica, a informação clássica (que pode ser expressa em bits) é codificada em propriedades de estados quânticos não ortogonais da luz. Assim, a codificação é feita de modo que a informação clássica fique protegida, permitindo que Alice e Bob gerem e compartilhem, de forma segura, sequências de chaves aleatórias \cite{bennett2014quantum, pirandola2020advances}. 

Um protocolo \gls{QKD} realiza a distribuição (ou geração) de chaves por meio da transmissão de estados quânticos por um canal quântico inseguro e do seu pós-processamento com o uso de um canal clássico autenticado (vide Figura~\ref{fig:cenarioQKD}). Neste contexto, o canal quântico representará o meio físico destinado exclusivamente ao envio dos estados quânticos. Já o canal clássico público autenticado consistirá em uma rede de telecomunicações convencional, embora este seja um meio público e permita a leitura dos dados, a sua autenticação garante que a espiã não consiga alterar as mensagens ou a identidade légitima. Assumimos que a espiã (Eva), por sua vez, tenha controle total sobre o canal quântico e seja capaz de observar toda a comunicação realizada pelo canal clássico autenticado~\cite{dias}. A segurança incondicional é garantida por propriedades de sistemas quânticos (e.g., superposição, emaranhamento) e por princípios da Mecânica Quântica, como o teorema da não-clonagem, que, em teoria, tornam impossível que Eva interfira na comunicação sem ser detectada~\cite{wolf}. 

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.6\linewidth]{images/cenarioQKD.pdf}
    \caption{Cenário de comunicação em QKD.}
    \label{fig:cenarioQKD}
\end{figure}

\subsection{Estrutura geral dos protocolos Prepara e Mede (P\&M)}

Podemos classificar os protocolos \gls{QKD} em duas categorias principais: o \gls{DV-QKD} e os baseados em \gls{CV-QKD} \cite{laudenbach2018continuous}. Essas duas famílias de protocolos diferem fundamentalmente na forma como a informação é codificada e detectada nos estados quânticos, o que acarreta implicações significativas em termos de implementação, custo, desempenho e maturidade de segurança~\cite{dias}. A Tabela~\ref{tab:compDVCV} apresenta as principais diferenças, vantagens e desvantagens de cada abordagem. 

\begin{table}[htpb]
\centering
\caption{Tabela comparativa entre protocolos DV e CV~\cite{tacla}}
\label{tab:compDVCV}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{|l|l|l|}
\hline
\textbf{Etapa} & \textbf{Variáveis Discretas} & \textbf{Variáveis Contínuas} \\
\hline
Codificação da chave & Polarização de fótons únicos & Quadraturas do campo \\
\hline
Detecção & Detecção de fóton único & Detecção homódina ou heteródina \\
\hline
Pós-processamento & Baixa complexidade & Quantização da chave e correção de erros com alta complexidade computacional \\
\hline
\end{tabular}
\end{adjustbox}
\end{table}

Os protocolos \gls{DV-QKD}, como o \gls{BB84}, utilizam sistemas quânticos discretos, como, por exemplo, fótons únicos com informação codificada em sua polarização, apresentando alta sensibilidade à temperatura dos fotodetectores e exigindo condições criogênicas para longas distâncias, o que torna tanto a transmissão quanto a detecção dessas partículas um desafio. Já os protocolos \gls{CV-QKD} utilizam estados do campo eletromagnético cujas variáveis (contínuas) carregam a informação, enquanto as detecções, tipicamente homódina ou heteródina, medem as quadraturas do campo~\cite{weedbrook, laudenbach} - uma das principais vantagens de utilizar sistemas \gls{CV-QKD} é a compatibilidade que eles têm com tecnologias de comunicações ópticas disponíveis comercialmente~\cite{dias}.  Vale destacar que, na prática, fontes perfeitas de fótons únicos ainda não estão disponíveis, e as implementações de protocolos DV consideram fontes emissoras de mais de um fóton, inclusive estados coerentes atenuados~\cite{pirandola}.  Contudo, os protocolos \gls{CV-QKD} demandam pós-processamento da chave, com códigos corretores de erro e funções de quantização, devido à modulação contínua aplicada~\cite{dias}. 

As etapas posteriores à comunicação quântica estão atreladas ao pós-processamento. Depois que Alice transmite e Bob mede os estados quânticos, o pós-processamento realiza a estimação de parâmetros, a correção de erros, a amplificação de privacidade e, finalmente, a obtenção da chave final. Essa chave, que é simétrica e compartilhada entre as partes, pode então ser utilizada para cifrar mensagens de forma segura – por exemplo, empregando o esquema de cifra de fluxo \gls{OTP}. Em resumo, o protocolo divide-se em quatro etapas principais, descritas na Figura~\ref{fig:protocolPEM}. 

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.6\linewidth]{images/protocolPEM.pdf}
    \caption{Representação esquemática das etapas de um protocolo de comunicação do tipo P\&M~\cite{tacla}.}
    \label{fig:protocolPEM}
\end{figure}

\begin{itemize}
    \item Distribuição de estados quânticos (Fase Quântica): Alice prepara e envia estados quânticos para Bob por meio de um canal quântico. 
    \item Estimação de parâmetros (Fase Clássica): Alice e Bob divulgam publicamente uma parte de suas sequências para estimar parâmetros do canal, como a transmitância e o ruído de excesso. 
    \item Reconciliação de chaves (correção de erros - Fase Clássica): Algoritmos de correção de erros são usados para garantir que Alice e Bob tenham sequências de bits idênticas.  
    \item Amplificação de privacidade (Fase Clássica): A chave comum é processada para garantir que seja estatisticamente independente da informação de Eva. 
\end{itemize}

A distribuição de estados pode ser realizada por dois modelos equivalentes para fins de análise de segurança: o modelo \gls{PM}, em que Alice prepara estados e os envia a Bob, e o modelo \gls{EB}, em que Alice e Bob compartilham estados emaranhados.  

Para superar os desafios de implementação e de pós-processamento~\cite{diamanti2016practical}, têm sido explorados os protocolos de \gls{DM-CVQKD}. Esses protocolos mantêm compatibilidade com equipamentos ópticos padrão, eliminando a necessidade de operações de quantização complexas. No entanto, essa simplificação na implementação acarreta consequências no desempenho e aumenta a complexidade da análise de segurança, principalmente devido à natureza não gaussiana da modulação\cite{dias}. 

Os sistemas CV-\gls{QKD} se destacam pela sua compatibilidade com as infraestruturas de redes ópticas~\cite{dias}. Os casos de uso de \gls{QKD} implementados abrangem diversos setores, que vão desde a segurança governamental até aplicações em saúde e em infraestrutura crítica. Na Tabela~\ref{tab:usecaseQKD} são apresentados, de forma resumida, os casos de uso da CV-\gls{QKD}, destacando em que setor foi aplicada, qual tecnologia de criptografia foi empregada e para qual finalidade.  


\begin{longtable}{|p{3cm}|p{4.5cm}|p{3.5cm}|p{5cm}|}
\caption{Resumo dos casos de uso de QKD em aplicações}
\label{tab:usecaseQKD} \\
\hline
\textbf{Setor} & \textbf{Caso de uso} & \textbf{Implementação} & \textbf{Objetivo principal} \\
\hline
\endfirsthead

\hline
\textbf{Setor} & \textbf{Caso de uso} & \textbf{Implementação} & \textbf{Objetivo principal} \\
\hline
\endhead

\hline
\endfoot

\hline
\endlastfoot

\textbf{Governo} &
Autenticidade de resultados eleitorais de 2007 em Genebra, Suíça &
AES-256, HMAC-SHA-256 &
Autenticidade dos resultados eleitorais durante a transmissão \\
\hline

\textbf{Bancário / Financeiro} &
\textit{Backup} para recuperação de desastres em uma empresa de gestão de ativos na Suíça &
AES-256 &
Aumentar a segurança de dados sensíveis de negócios e clientes, garantindo sigilo futuro (forward secrecy) e protegendo contra futuras tentativas de descriptografia \\
\hline

\textbf{Bancário / Financeiro} &
A Toshiba e a \textit{Quantum Xchange} protegeram uma conexão entre os mercados financeiros de Wall Street e um data center em Nova Jersey &
AES &
Proteger a transmissão de dados financeiros sensíveis, como algoritmos de negociação, contas de clientes e dados de transações em tempo real \\
\hline

\textbf{Criptomoeda / Financeiro} &
Uma empresa na Suíça (\textit{Mt. Pelerin}) usou QKD da \textit{ID Quantique} para criptografar as “partes” de chaves privadas de \textit{blockchain} &
QKD (\textit{ID Quantique}), OTP\textsuperscript{4}, SSS\textsuperscript{5} &
Proteger o \textit{backup} e armazenamento de chaves privadas de ativos digitais, que são o alvo principal em ataques a criptomoedas \\
\hline

\textbf{Saúde / Pesquisa médica} &
Compartilhamento de imagens médicas e dados genéticos entre um centro de pesquisa e um hospital em Graz, Áustria, com armazenamento em \textit{data centers} externos &
As imagens foram divididas em três partes, e duas delas foram criptografadas com AES e QKD (\textit{ID Quantique}, Toshiba) antes de serem enviadas a \textit{data centers} diferentes &
Garantir a confidencialidade e integridade de dados médicos altamente sensíveis durante a transmissão entre hospitais e locais de armazenamento externos \\
\hline

\textbf{Saúde / Pesquisa médica} &
\textit{Backup} de registros médicos em uma instituição médica no Japão &
QKD (Rede QKD de Tóquio com equipamentos NEC, Toshiba, etc.), AONT\textsuperscript{6} &
Proteger a transmissão de registros médicos que contêm informações detalhadas e confidenciais de pacientes, protegendo-os contra perda de dados e acesso não autorizado \\
\hline

\textbf{Saúde / Pesquisa médica} &
Transmissão segura de dados de sequenciamento de genoma em larga escala e videoconferências entre um centro de análise e uma organização médica no Japão &
Sistema QKD (Toshiba) com criptografia OTP &
Garantir confidencialidade de longo prazo para dados genômicos, que são informações identificação pessoal e sensíveis \\
\hline

\textbf{Saúde / Pesquisa médica} &
Instituições na Espanha e em Portugal usaram QKD para calcular as distâncias evolutivas entre sequências de genomas sem revelar as sequências em si &
QKD com criptografia OTP &
Permitir o cálculo e compartilhamento seguro de distâncias genômicas para análises filogenéticas, sem expor os dados brutos \\
\hline

\textbf{Serviços Públicos / Energia} &
Uma empresa de serviços públicos suíça (SIG) usou QKD para proteger a conexão entre seus dois principais data centers &
QKD (\textit{ID Quantique}) e criptografia AES-256 &
Aumentar a segurança dos dados de operações de serviços públicos e informações de clientes processados em suas aplicações em nuvem \\
\hline

\textbf{Energia / Smart Grid} &
A IDQ e a SIG conectaram duas de suas estações de energia a um \textit{testbed OpenQKD} para demonstrar uma rede \textit{Smart Grid}, com o objetivo de proteger a transmissão de dados e detectar intrusões &
QKD (\textit{Qubitekk}, baseado em entrelaçamento), AES, GMAC\textsuperscript{7} &
Prevenir que \textit{hackers} assumam o controle da rede de distribuição de eletricidade, garantindo a transmissão segura de dados entre as estações de energia \\
\hline

\textbf{Energia / Smart Grid} &
Um sistema QKD foi implantado em uma distância de 3,4 km entre um centro de distribuição de energia e uma subestação elétrica nos EUA para autenticar o tráfego SCADA (dados de controle e medição) &
QKD (\textit{Qubitekk}), GMAC, AES &
Garantir a autenticidade do tráfego SCADA, que contém dados de controle e medição não confidenciais, como tensão e corrente, para proteger a infraestrutura crítica \\
\hline

\textbf{Automotivo} &
Pesquisadores na Rússia integraram \textit{hardware} QKD em um carro autônomo para trocar chaves com estações de recarga &
QKD (\textit{QRate}), as chaves foram usadas para estabelecer uma conexão \textit{OpenVPN} segura (via 4G LTE) com o data center do fornecedor &
Proteger a transferência e atualizações de \textit{software} remotas e dados de telemetria, prevenindo o acesso não autorizado ou a alteração do \textit{software} do sistema de controle autônomo \\
\hline

\end{longtable}

Apesar de a \gls{QKD} ter sido implementada em diversos cenários, como visto na Tabela~\ref{tab:usecaseQKD}, sua viabilidade como solução autônoma é limitada a casos específicos. Uma das limitações práticas da \gls{QKD} diz respeito ao seu desempenho reduzido em longas distâncias, especialmente em redes de fibra ótica~\cite{zeng}. Com o uso de fibras ópticas padrão, a \gls{SKR} tende a diminuir à medida que a distância aumenta. Isso ocorre porque a maioria dos fótons (que carregam as informações quânticas) é espalhada e absorvida ao longo da fibra antes mesmo de chegar ao receptor~\cite{zeng, quantropi}. Apenas 10\% dos fótons conseguem viajar mais de 50 quilômetros, e apenas 0,01\% ultrapassam 200 quilômetros~\cite{quantropi}. Migrar para \gls{QKD} pode ser uma tarefa complexa em termos de escala e custo, devido à sua implementação. Isso porque a implementação da \gls{QKD} exige hardware especializado, o que implica alto custo de implementação e a necessidade de grandes mudanças na infraestrutura para empresas que dependem de cabeamento padrão — que é econômico para comunicações internas~\cite{del, quantropi}. Além disso, a \gls{QKD} não possui autenticação integrada; ou seja, ela resolve o problema de distribuição de chave secreta, mas depende de autenticação na comunicação clássica para gerar a chave. Isso implica uma possível vulnerabilidade a ataques do tipo \gls{MitM}, em que um hacker se comunica com as partes sem o seu conhecimento (o que ocorre se não houver um mecanismo de autenticação)~\cite{le}. Desse modo, os protocolos \gls{QKD} devem ser complementados por medidas criptográficas clássicas que autentiquem a fonte da transmissão~\cite{quantropi}. 

De acordo com os casos de uso apresentados na Tabela~\ref{tab:usecaseQKD}, percebe-se que a distribuição quântica de chaves é adequada para troca segura de chaves em setores críticos, como serviços financeiros, redes de telecomunicações essenciais e aplicações de defesa. Entretanto, as limitações citadas acima podem restringir sua praticidade em qualquer setor. Apesar de suas limitações, a \gls{QKD} ainda é uma tecnologia relevante e promissora no cenário de proteção contra ameaças quânticas, devido à sua base teórica de segurança. 


\section{Visão geral da pilha \gls{TCP/IP}}

A arquitetura \gls{TCP/IP} organiza os protocolos de comunicação em camadas, nas quais cada uma desempenha funções específicas e se comunica com as camadas adjacentes. Esse modelo facilita a interoperabilidade, a modularidade e a evolução independente dos protocolos. A pilha \gls{TCP/IP} é composta por quatro camadas principais: aplicação, transporte, internet e acesso à rede. Na Figura~\ref{fig:protocols}, observa-se a presença de protocolos típicos dessas camadas, como TLS/HTTPS, TCP/UDP, IP e Ethernet, além de mecanismos de segurança que atuam em diferentes níveis da pilha. 

\begin{figure}[ht]
    \centering
    \includegraphics[width=1\linewidth]{images/protocols.pdf}
    \caption{Protocolos de segurança no modelo \gls{TCP/IP}.}
    \label{fig:protocols}
\end{figure}

A camada de aplicação é a mais próxima do usuário e define os protocolos utilizados diretamente pelas aplicações para comunicação na rede. Na Figura~\ref{fig:protocols}, vê-se o uso de TLS/HTTPS, em que o \gls{HTTPS} corresponde à versão segura do protocolo HTTP. O \gls{TLS} é responsável por garantir a autenticação das partes, a confidencialidade e a integridade dos dados transmitidos. Esse protocolo atua criptografando as informações da aplicação antes de entregá-las à camada de transporte, garantindo que o conteúdo não possa ser interpretado por intermediários ao longo do caminho~\cite{peterson2007computer}. 

A camada de transporte é responsável pela comunicação fim a fim entre aplicações em \textit{hosts} diferentes. Nessa camada, a Figura~\ref{fig:protocols} apresenta os protocolos \gls{TCP} e \gls{UDP}. O \gls{TCP} é orientado à conexão e oferece mecanismos de confiabilidade, como garantia de entrega, controle da ordem dos pacotes e controle do fluxo e do congestionamento. Por isso, é utilizado por aplicações que necessitam de comunicação confiável, como \gls{HTTPS}, \gls{SSH} e serviços de e-mail. Já o \gls{UDP} é um protocolo não orientado à conexão, que não garante entrega nem ordem dos pacotes, mas apresenta menor latência e menor sobrecarga, sendo comum em aplicações de tempo real, como \textit{streaming}, voz sobre \gls{IP}, jogos online e \gls{DNS}. A aplicação pode escolher entre \gls{TCP} ou \gls{UDP} conforme os requisitos do serviço~\cite{peterson2007computer}. 

A camada de internet é responsável pelo endereçamento lógico e pelo roteamento de pacotes entre redes distintas. O principal protocolo dessa camada é o \gls{IP}, cuja função é identificar os dispositivos por meio de endereços lógicos e encaminhar os pacotes ao destino correto. O \gls{IP} não garante a entrega nem a ordem dos pacotes, delegando essas responsabilidades à camada de transporte, especialmente ao \gls{TCP}. Na figura, o \gls{IP} encapsula os dados provenientes do \gls{TCP} ou do \gls{UDP} e os envia pela rede até o destino~\cite{peterson2007computer}. 

A camada de acesso à rede, também chamada de camada de enlace, é responsável pela comunicação local entre dispositivos conectados ao mesmo meio físico. Na Figura~\ref{fig:protocols}, apresenta-se o protocolo Ethernet, que utiliza endereços \gls{MAC} para identificar os dispositivos no enlace local e encapsular os dados em quadros. Um ponto importante a ser ilustrado é que os endereços \gls{MAC} mudam a cada salto entre \textit{switches}, pois são válidos apenas em um segmento de rede. Em contraste, o endereço \gls{IP} permanece o mesmo ao longo de todo o trajeto fim a fim~\cite{peterson2007computer}. 

A Figura~\ref{fig:protocols} também destaca diferentes pontos da pilha onde a criptografia pode ser aplicada. No nível da aplicação, o TLS/HTTPS protege os dados entre as aplicações dos \textit{hosts}. Nesse caso, mesmo que os pacotes sejam interceptados durante o percurso, o conteúdo da aplicação permanece cifrado e ilegível aos intermediários. 

Outro mecanismo ilustrado é o uso de túneis \gls{VPN}, como \gls{IPsec} ou WireGuard, que operam na camada de rede. Nesse cenário, é criado um túnel criptografado entre \textit{gateways}, encapsulando o pacote original dentro de um novo pacote \gls{IP}. O conteúdo interno, incluindo cabeçalhos \gls{IP}, TCP/UDP, \gls{TLS} e dados da aplicação, permanece protegido durante o trânsito. Assim, a rede intermediária só consegue visualizar o cabeçalho externo do túnel, sem acesso ao conteúdo da comunicação. 

Por fim, a Figura~\ref{fig:protocols} mostra a criptografia na camada de enlace, que protege apenas a comunicação entre dois dispositivos diretamente conectados. Nesse modelo, cada enlace possui sua própria criptografia, e os dados podem ser descriptografados e recriptografados a cada salto. Isso significa que a proteção é local e não fim a fim, diferentemente do \gls{TLS} ou de túneis \gls{VPN}. 


% \section{Protocolos de comunicação}

% Nesta seção, são descritos protocolos de comunicação de segurança comumente aplicados em diferentes camadas da rede.

% \subsection{\gls{TLS}}

% A \gls{TLS} é um protocolo de comunicação que evolui do antigo \gls{SSL}, renomeado após a versão 3.0 do \gls{SSL} e apoiado pela \gls{IETF}.

% O \gls{TLS} opera entre duas entidades, nomeadas cliente e servidor, na camada de transporte \gls{TCP}, garantindo a confidencialidade, a integridade e a autenticidade dos dados transmitidos. O \gls{TLS} é composto por uma série de etapas.

% A etapa de \textit{handshake} envolve a troca de mensagens entre o cliente e o servidor para iniciar a comunicação criptografada. A primeira mensagem é enviada pelo cliente, incluindo a versão do \gls{TLS} suportada, os algoritmos de chave pública, entre outros parâmetros. O servidor retorna a mensagem indicando a versão de \gls{TLS} selecionada, o algoritmo de criptografia e o algoritmo de chave pública a serem utilizados, e fornece um certificado digital contendo a chave pública do servidor. 

% Na etapa de autenticação e troca de chaves, o cliente verifica a autenticidade do certificado recebido. Se necessário, verifica a cadeia de certificação até uma autoridade certificadora confiável. O cliente gera uma chave de sessão e a criptografa com a chave pública do servidor para enviá-la ao servidor. Com sua chave privada, o servidor consegue descriptografar a chave de seção gerada pelo cliente.

% Por fim, o cliente envia uma mensagem ao servidor indicando que as mensagens futuras serão criptografadas com a chave de sessão compartilhada~\cite{rfctls1.3}.


% \subsection{\gls{IPsec}}

% O \gls{IPsec} é um conjunto de protocolos de segurança desenvolvido pela \gls{IETF} com o objetivo de garantir confidencialidade, integridade, autenticação e proteção contra ataques de repetição no tráfego IP. Diferentemente de protocolos como o \gls{TLS}, que operam na camada de transporte, o \gls{IPsec} atua diretamente na camada de rede do modelo TCP/IP, podendo proteger qualquer protocolo de camada superior de forma transparente às aplicações.

% O \gls{IPsec} pode operar em dois modos: modo transporte e modo túnel. No modo transporte, apenas o payload do pacote IP é protegido, mantendo o cabeçalho IP original. Já no modo túnel, todo o pacote IP é encapsulado em um novo pacote, fornecendo proteção completa entre \textit{gateways} ou entre um cliente e um \textit{gateway}, cenário típico de \gls{VPN}.

% O estabelecimento de uma comunicação segura em \gls{IPsec} é realizado por meio do protocolo \gls{IKE}, responsável por negociar parâmetros criptográficos, autenticar os pares e estabelecer \gls{SA}. Esse processo ocorre em fases. Na primeira fase, chamada IKE SA, os pares negociam algoritmos de hash, de criptografia e de autenticação, além de estabelecer um canal protegido para a fase seguinte. Na segunda fase, denominada IPsec SA, são negociados os parâmetros específicos para proteger o tráfego dos protocolos \gls{AH} e \gls{ESP}.

% A troca de chaves no \gls{IKE} utiliza, tipicamente, o método de Diffie–Hellman, permitindo o estabelecimento de chaves simétricas de sessão de forma segura, mesmo em canais não confiáveis. A autenticação entre os pares pode ocorrer por meio de certificados digitais, \gls{PSK} ou métodos baseados em \textit{tokens}.

% O \gls{IPsec} oferece dois protocolos principais para proteção do tráfego: o \gls{AH} e o \gls{ESP}. O \gls{AH} provê autenticação e integridade do pacote, mas não oferece confidencialidade. Já o \gls{ESP}, protocolo mais amplamente utilizado, oferece confidencialidade, autenticação, integridade e proteção contra \textit{replay attacks}. Após a negociação das \gls{SA}, todo o tráfego protegido é processado conforme os parâmetros definidos durante a troca de chaves, garantindo segurança fim a fim ou entre pontos específicos da rede~\cite{rfcipsec}.

==> tex/integration.tex <==
\chapter{Técnicas para integração clássico-QKD}
\label{chapter:integration}

Nesta seção, apresentaremos as abordagens de integração entre sistemas \gls{QKD} e redes de computadores descritas na literatura. O objetivo da busca por essas técnicas de integração é identificar como sistemas \gls{QKD} podem ser utilizados nas diferentes camadas do modelo OSI. Além disso, analisamos trabalhos que utilizam técnicas presentes em redes de computadores para facilitar e expandir o funcionamento de sistemas QKD, como, por exemplo, o SDN, o KMS, a abstração e a virtualização de QKD em camadas independentes, entre outras.

\section{Padronização e especificações}

Atualmente, existem documentos de especificação relacionados ao QKD \cite{etsiqkd004} em desenvolvimento e com versões já disponíveis de entidades de padronização, como a \gls{ETSI} e a \gls{ITU}, entre outras.

Entre os documentos definidos pela \gls{ETSI} estão os protocolos \cite{lucamarini} e formatos de dados para entrega de chaves \gls{QKD} por meio de uma API REST. O objetivo principal é padronizar a interface entre aplicações e a rede \gls{QKD}, permitindo interoperabilidade entre equipamentos de diferentes fabricantes. 

O padrão ETSI GS QKD 014~\cite{etsiqkd014} descreve a comunicação entre a \gls{SAE}, que utiliza as chaves, a \gls{KME}, responsável por gerar e entregar as chaves, e a rede \gls{QKD}, responsável por gerar e distribuir as chaves entre os \gls{KME}. O documento define uma API REST baseada em \gls{HTTPS}, com formato de requisições e respostas em \gls{JSON}.

Outra especificação publicada pela \gls{ETSI} é o documento ETSI GS QKD 004~\cite{etsiqkd004}. Esse documento também define uma API entre as aplicações e a camada de gerenciamento de chaves. O objetivo é que aplicações em dois pontos da rede recebam, de forma controlada, fluxo de chaves simétricas idênticas, geradas por \gls{QKD}. O documento define que o QKD \gls{KM} gerencie as chaves geradas pelo QKD, sincronize as chaves entre os dois lados da comunicação e entregue conjuntos idênticos de chaves às duas partes. Diferentemente do ETSI GS QKD 014, que segue o modelo de requisição/resposta, a interface é orientada por sessões, nas quais a aplicação consome chaves continuamente. Nessa especificação há suporte a \gls{QoS}, permitindo especificar a taxa mínima de geração de chaves, prioridade, entre outros parâmetros.

\section{KMS}

% Explicar o que é, citar exemplos. 
% Usar as referência que temos para explicar o que estamos escrevendo, não para explicar o trabalho específico.

% E.g KMS são usados em QKD com nodos confiáveis... Citar os trabalhos sobre isso aqui
Um \gls{KMS} é um sistema responsável por gerar, armazenar, distribuir, rotacionar e destruir chaves criptográficas utilizadas por aplicações e serviços. Ele é um componente central em arquiteturas de segurança, pois garante o uso de criptografia de forma controlada, auditável e segura. Em vez de cada aplicação gerenciar suas próprias chaves, o \gls{KMS} atua como uma entidade confiável que fornece chaves sob demanda, aplicando políticas de acesso, autenticação e controle de ciclo de vida.

A principal responsabilidade de um \gls{KMS} é o gerenciamento do ciclo de vida das chaves criptográficas. Isso inclui a geração segura de chaves, seu armazenamento em ambientes protegidos (como \gls{HSM}), a distribuição controlada para aplicações autorizadas e, por fim, a revogação ou destruição das chaves quando não forem mais necessárias. Além disso, o \gls{KMS} é responsável por tarefas como a rotação periódica de chaves, o versionamento e a auditoria de uso, o que ajuda a reduzir o impacto de eventuais comprometimentos.

O funcionamento de um \gls{KMS} normalmente segue um modelo cliente-servidor. As aplicações, chamadas de clientes, solicitam operações criptográficas ou chaves ao \gls{KMS} por meio de uma API. O \gls{KMS} verifica a identidade da aplicação, suas permissões e as políticas de segurança associadas. Se a requisição for autorizada, o sistema fornece a chave solicitada ou realiza a operação criptográfica em nome da aplicação. Em muitos sistemas modernos, as chaves sensíveis nunca deixam o ambiente seguro do \gls{KMS}; em vez disso, o próprio \gls{KMS} executa operações como criptografia, descriptografia e assinatura digital.

Além do controle de acesso, um \gls{KMS} também desempenha um papel importante na segurança operacional e na conformidade. Ele mantém registros de auditoria detalhados sobre quem utilizou cada chave, quando e para que finalidade. Esses registros são essenciais para atender aos requisitos regulatórios e investigar incidentes de segurança. O \gls{KMS} também permite a definição de políticas, como restrições de uso por aplicação, limites de validade ou exigência de múltiplos fatores de autenticação para operações críticas.

Em sistemas que utilizam \gls{QKD}, o \gls{KMS} desempenha uma função adicional: atua como a entidade responsável por gerenciar e sincronizar as chaves geradas pelos dispositivos \gls{QKD} e por entregá-las às aplicações. Nesse contexto, o \gls{KMS} garante que ambos os lados da comunicação recebam conjuntos idênticos de chaves, além de controlar parâmetros como a qualidade de serviço, a taxa de geração de chaves e o tempo de vida dessas chaves. Dessa forma, ele atua como uma camada intermediária entre os equipamentos \gls{QKD} e as aplicações que consomem as chaves.

% Talvez poderia trazer em algum momento como são essas propostas
% Como isso ainda está sendo desenvolvido, é possível especificar os tipos de KMS, como eles são. Como não deve ter um padrão, dá para mostrar as diferentes abordagens. Como se divide em camada, como é implementado.

A partir da literatura, foi possível perceber como o uso de \gls{KMS} pode aprimorar o uso das chaves geradas por um sistema \gls{QKD}. Abstrair a camada de gerenciamento de chaves, afastando-a do hardware, melhora a flexibilidade, a interoperabilidade e o desempenho, além de permitir a customização de mecanismos como \gls{QoS}~\cite{1.4}~\cite{1.70}. O uso de \gls{KMS}, combinado com tecnologias como \gls{SDN}, também pode auxiliar no estabelecimento de redes com nós confiáveis e \textit{multi-hops}; em larga escala, pode beneficiar o gerenciamento da rede, com redundância, alta disponibilidade, balanceamento de carga, entre outros~\cite{1.24}~\cite{1.26}~\cite{1.50}. O uso de \gls{KMS} também traz uma perspectiva mais virtual ao \gls{QKD}, possibilitando a entrega de chaves como serviço e criando \textit{frameworks} que facilitam o uso dessas chaves em sistemas nativos na nuvem~\cite{1.40}~\cite{1.80}.

\section{SDN}

\gls{SDN} é um paradigma de redes que separa as funções de controle e de encaminhamento de dados em uma infraestrutura de comunicação~\cite{1.50}. Em redes tradicionais, os dispositivos de rede, como roteadores e \textit{switches}, tomam decisões de encaminhamento localmente, com base em suas próprias tabelas de roteamento e em protocolos distribuídos. No \gls{SDN}, essa lógica de controle é centralizada em um componente chamado controlador, enquanto os dispositivos de rede passam a executar apenas a função de encaminhar pacotes conforme as regras de encaminhamento recebidas. O plano de controle é acoplado ao \textit{switch}/roteador, portanto, decisões de roteamento são tomadas através de protocolos distribuídos de diferentes \textit{switches}.

A principal ideia por trás do \gls{SDN} é tornar a rede programável e flexível. O controlador \gls{SDN} mantém uma visão global da rede e define políticas de encaminhamento, qualidade de serviço, segurança e priorização de tráfego. Essas políticas são, então, aplicadas aos dispositivos de rede por meio de protocolos padronizados, como o \textit{OpenFlow}. Esse protocolo permite que as mudanças na rede sejam feitas de forma centralizada, por meio de software, sem a necessidade de configurar manualmente cada equipamento.

O \gls{SDN} gerencia o plano de controle de forma centralizada. O controlador é responsável por calcular rotas, aplicar políticas de segurança, gerenciar o congestionamento, balancear a carga e adaptar o comportamento da rede às necessidades das aplicações. Como ele possui uma visão global da topologia e do estado da rede, pode tomar decisões mais eficientes e coerentes do que dispositivos operando de forma independente.

O funcionamento de uma rede \gls{SDN} geralmente é dividido em três camadas. O plano de dados é composto por dispositivos de rede, como \textit{switches} e roteadores, responsáveis apenas pelo encaminhamento de pacotes. A camada de controle é composta pelo controlador \gls{SDN}, que contém a lógica de decisão e de gerenciamento da rede. Por fim, a camada de aplicação contém softwares e serviços que utilizam a rede e definem políticas, como sistemas de monitoramento, balanceadores de carga, mecanismos de segurança e aplicações de orquestração.

A comunicação entre essas camadas ocorre por meio de interfaces padronizadas. A interface entre o controlador e os dispositivos de rede é chamada de \textit{southbound interface}, e o \textit{OpenFlow} é um dos protocolos mais conhecidos. Já a interface entre o controlador e as aplicações é chamada de \textit{northbound interface}, normalmente implementada por meio de APIs que permitem às aplicações programar o comportamento da rede.

Em contextos avançados, como redes ópticas ou redes integradas à criptografia quântica, o \gls{SDN} pode ser utilizado para orquestrar recursos de comunicação e de segurança. Por exemplo, o controlador \gls{SDN} pode selecionar rotas que suportem enlaces \gls{QKD}, gerenciar a distribuição de chaves ou adaptar o comportamento da rede à disponibilidade de chaves seguras. Dessa forma, o \gls{SDN} atua como o elemento de inteligência e automação que integra diferentes tecnologias de rede em uma arquitetura unificada.

A utilização de \gls{SDN} para controlar, gerenciar e orquestrar sistemas \gls{QKD} integrados ao clássico tem se tornado necessária para garantir a interoperabilidade das redes e permitir o controle remoto e programável dos dispositivos \gls{QKD}. É possível utilizar \gls{SDN} para integrar o \gls{QKD} à infraestrutura óptica, gerenciar a coexistência com canais clássicos e alocar recursos~\cite{1.3}~\cite{1.17}. O \gls{SDN} pode ainda ser utilizado para controlar outros aspectos relacionados à comunicação \gls{QKD}, como, por exemplo, a autenticação entre nós \gls{QKD}~\cite{1.23}.

\section{Sumário da literatura}

% Apresentar uma tabela com os trabalhos selecionados

% Talvez se fizer sentido, colocar uma seção anterior falando sobre a metodologia da busca.

% Criar uma subseção para cada técnica e agrupar os artigos nessas subseções.

A Tabela~\ref{tab:rev_literatura} apresenta uma síntese dos principais resultados encontrados. Além dos trabalhos que propõem arquiteturas e modelos para a integração de \gls{QKD} com redes clássicas, principalmente por meio de \gls{KMS} e \gls{SDN}, também selecionamos trabalhos que implementam modificações nos protocolos de segurança de rede, como \gls{TLS} e \gls{IPsec}, que permitam a utilização de chaves \gls{QKD} nesses protocolos. 

\begin{longtable}{|p{5cm}|p{3cm}|p{6cm}|}
\caption{Sumário da revisão da literatura}
\label{tab:rev_literatura} \\

\hline
\textbf{Artigo} & \textbf{Categoria} & \textbf{Observações} \\ \hline
\endfirsthead

\hline
\textbf{Artigo} & \textbf{Categoria} & \textbf{Observações} \\ \hline
\endhead

\hline
\endfoot

\hline
\endlastfoot

Unleashing flexibility and interoperability in QKD networks: The power of softwarized architectures \cite{1.4} 
& \gls{KMS} & Propõe um modelo de KMS desagregado suportado por vitualização e softwarização. Facilita o controle e o acesso à rede \gls{QKD}. \\ \hline

Toward quantum-safe scalable networks: an open, standards-aware key management framework \cite{1.24} 
& \gls{KMS} e \gls{SDN} & Propõem uma arquitetura de rede que resolve desafios do \gls{KMS}, como identificação, retransmissão, descoberta de caminhos e escalabilidade, por meio do uso de \gls{SDN}. \\ \hline

DISCRETION: First Field Demonstration of a Quantum Enabled SDN in the Context of a Military Exercise \cite{1.26} 
& \gls{KMS} e \gls{SDN} & Possui uma implantação prática de uma rede baseada em \gls{SDN}, na qual o \gls{QKD} é incorporado para garantir alta segurança criptográfica.  \\ \hline

KaaS: Key as a service over quantum key distribution integrated optical networks \cite{1.40} 
& \gls{KMS} & Propõe um \textit{framework} para a entrega de chaves como serviço, facilitando a implantação e o uso de chaves em redes ópticas integradas com \gls{QKD}. \\ \hline

Quantum aware SDN nodes in the Madrid quantum network \cite{1.50} 
& \gls{SDN} & Relata aspectos da implantação da rede quântica de Madrid, com base em \gls{SDN}. Nessa implantação, o SDN é usado para integrar e gerenciar canais clássicos e quânticos. Também são analisados aspectos de segurança relacionados ao plano de controle do \gls{SDN}, uma vez que se trata de uma infraestrutura crítica nesse cenário. \\ \hline

Network Slicing-Based and QoS-Oriented Software-Defined Quantum Key Distribution Network \cite{1.70} 
& \gls{SDN} e \gls{QoS} & Propõem uma arquitetura orientada a \gls{QoS} baseada em fatiamento de rede e em \gls{SDN}. O fatiamento da rede, somado ao \gls{QoS}, pode atender a diferentes demandas, de acordo com os requisitos do usuário. Os resultados simulados mostram a flexibilidade e a facilidade de integrar os serviços orquestrados em redes de comunicação existentes. \\ \hline

An Enhanced Virtualized Control and Key Management Model for QKD Networks \cite{1.80} 
& \gls{KMS} & Os autores apresentam um modelo operacional para redes \gls{QKD}, virtualizando funcionalidades de controle e de gerenciamento de chaves. A virtualização permite abstrair recursos de hardware, tornando mais fácil gerenciar e escalar de forma dinâmica.  \\ \hline

Continuous variable QKD in flexible optical networks for future quantum secure connectivity \cite{1.3} 
& \gls{SDN} & Os autores combinam análise de segurança, simulações de coexistência com tráfego clássico e aspectos de controle via \gls{SDN} para demonstrar como o \gls{CV-QKD} pode ser integrado a redes ópticas modernas. \\ \hline

Software-defined control of integrated QKD and classical optical networks \cite{1.17} 
& \gls{SDN} & O artigo propõe um \textit{framework} de controle baseado em \gls{SDN} para integrar redes ópticas clássicas e \gls{QKD}. O controlador \gls{SDN} é capaz de orquestrar dispositivos ópticos e nós \gls{QKD}, permitindo o registro de aplicações, a criação dinâmica de enlaces quânticos e a distribuição de chaves. \\ \hline

Enabling PUF-based Authentication in QKD Networks \cite{1.23} 
& \gls{SDN} e Autenticação \gls{QKD} & Os autores propõem e demonstram um mecanismo de autenticação de nós \gls{QKD} baseado em \gls{PUF}, integrado a um \textit{framework} de controle \gls{SDN} padronizado. A solução utiliza a assinatura física única da fibra óptica para autenticar os nós antes da geração de chaves e implementa esse processo em um fluxo automatizado de ativação de enlaces quânticos. \\ \hline

Towards a quantum-safe 5G: Quantum Key Distribution in core networks \cite{3.1} 
& Integração com protocolos de segurança & O artigo propõe e implementa um sistema para tornar o core de redes 5G \textit{quantum-safe}, integrando \gls{QKD} ao protocolo \gls{TLS} utilizado entre as funções de rede. A solução usa chaves geradas por \gls{QKD} para autenticação e criptografia entre as funções do \textit{core}, com um repositório central de chaves \\ \hline

Integrating quantum key distribution into tls 1.3: A transport layer approach to quantum-resistant communications in optical networks \cite{3.2} 
& Integração com protocolos de segurança & O artigo apresenta uma implementação experimental de \gls{TLS} 1.3 resistente a ataques quânticos, integrando \gls{QKD} ao processo de troca de chaves em um ambiente óptico. A solução combina \gls{QKD} com criptografia clássica no \textit{handshake}. \\ \hline

Quantum-resistant transport layer security \cite{3.3} 
& Integração com protocolos de segurança & O artigo propõe e implementa um \gls{TLS} resistente a ataques quânticos, combinando \gls{QKD} e \gls{PQC} no processo de \textit{handshake}. Ele apresenta duas formas de integrar as chaves (concatenação e XOR), implementa a solução em um ambiente experimental com dispositivos reais e avalia o impacto no desempenho e na segurança, mostrando que o modelo híbrido aumenta a segurança ao custo de maior tempo de estabelecimento de chaves. \\ \hline

VPN protection with QKD-derived keys using standard interfaces \cite{3.4} 
& Integração com protocolos de segurança & O artigo propõe uma arquitetura de \gls{VPN} protegida por chaves derivadas de \gls{QKD}, integrando dispositivos de \gls{QKD} ao OpenVPN por meio de interfaces padronizadas (ETSI GS QKD 004~\cite{etsiqkd004}). A solução utiliza um aplicativo intermediário para obter chaves do sistema \gls{QKD} e configurá-las automaticamente no túnel \gls{VPN} \\ \hline

Quantum secured internet transport \cite{3.5} 
& Integração com protocolos de segurança & Os autores propõem e demonstram um sistema de transporte seguro para a Internet baseado em \gls{QKD}, integrando as chaves do sistema \gls{QKD} ao protocolo \gls{TLS} por meio de um modelo de chaves pré-compartilhadas e \textit{proxies} transparentes para aplicações existentes. A solução é validada em um protótipo com enlaces \gls{QKD} entre dois ambientes e distribuição local de chaves, mostrando como serviços comuns (web, vídeo, chat) podem operar sobre um túnel \gls{TLS} protegido por \gls{QKD}. \\ \hline

Uma Abordagem para Prototipagem de Aplicações com Distribuição Quântica de Chaves \cite{3.6} 
& Integração com protocolos de segurança & O artigo propõe uma plataforma de prototipagem de aplicações baseadas em \gls{QKD} por meio de co-simulação entre um simulador quântico (NetSquid) e um emulador de rede clássica (Mininet), integrados por um \textit{gateway} e por um sistema de gerenciamento de chaves. Como prova de conceito, a solução demonstra comunicação segura entre hosts usando \gls{IPsec} com chaves geradas por \gls{QKD}, permitindo testar integrações quântico-clássicas sem necessidade de hardware físico. \\ \hline

\end{longtable}

Apesar dos avanços já apresentados pelos autores e do desenvolvimento inicial dos padrões de interfaces de comunicação para sistemas \gls{QKD}, é necessário continuar investigando a integração de redes clássicas com técnicas de segurança que sejam resistentes a ataques quânticos, para garantir um modelo de rede seguro contra ataques quânticos.

\section{Integração com o modelo \gls{TCP/IP}}

Analisamos agora os protocolos de comunicação sob a ótica do nível de abstração (por exemplo, camadas do \gls{TCP/IP}) em que as técnicas criptográficas investigadas operam, considerando os domínios clássicos ou clássicos/quânticos. Também consideramos brevemente trabalhos que propõem segurança pós-quântica com base em \gls{PQC}, pois, em muitos casos, indicam percepções relacionadas à \gls{QKD} ou até mesmo adotam um uso "híbrido" para garantir segurança e, por vezes, redundância.

\subsection{Implantações nas camadas do \gls{TCP/IP}}

Diversas iniciativas de comunicação segura já incorporam algoritmos resilientes a ataques quânticos. A integração de \gls{PQC} e \gls{QKD} abrange múltiplas camadas do modelo clássico \gls{TCP/IP}, variando desde camadas inferiores, como a camada de enlace de dados, até a camada de aplicação. Esse é o domínio em que ambas as abordagens investigadas aparecem com maior frequência na literatura. A seguir, analisamos tais iniciativas de forma top-down, da camada de aplicação até a camada de enlace de dados.

\textbf{Camada de Aplicação.}
A camada de aplicação fornece uma interface direta com os usuários e a rede. Protocolos alternativos incluem soluções de acesso remoto seguro, como \gls{SSH}, e protocolos \textit{publish–subscribe}, como \gls{MQTT}, comumente utilizados em sistemas de \gls{IoT} \cite{malina2024quantum}. O \gls{TLS}, base da navegação web moderna, também está passando por atualizações. Versões recentes do \gls{TLS} incorporam \gls{PQC} tanto para autenticação quanto para criptografia. De forma semelhante, o QUIC, que é uma alternativa à pilha tradicional TCP/TLS, também vem sendo alvo de integração com primitivas resistentes a ataques quânticos \cite{kempf2024quantum}. O QUIC combina os handshakes do \gls{TLS} e do \gls{TCP}, reduzindo o tempo de ida e volta necessário para o estabelecimento de conexões, o que o torna adequado para aplicações que exigem baixa latência. Esforços para incluir \gls{QKD} no \gls{TLS} também são encontrados na literatura \cite{garcia2023quantum}, mas, devido à sua complexidade e ao custo, ainda não há adoção em larga escala.

Aplicações de troca de mensagens ponta a ponta, como e-mail e mensagens instantâneas, devem garantir proteção contra interceptação. Esses são exemplos de aplicações-alvo para a integração de \gls{PQC} \cite{847_doberl2023quantum}. Embora o e-mail tradicionalmente dependa de protocolos como o \gls{SMTP}, a criptografia ponta a ponta pode ser implementada no nível da aplicação, garantindo que apenas o remetente e o destinatário possam descriptografar a mensagem. Um exemplo é o protocolo \textit{Signal} com \textit{Triple Ratchets} \cite{dodis2025triple}. É importante observar que a criptografia ponta a ponta difere de outras formas de segurança em nível de protocolo na camada de aplicação, nas quais intermediários (por exemplo, servidores centralizados) ainda podem ter acesso ao conteúdo das mensagens.

Outro caso de uso de criptografia ponta a ponta é o uso do \gls{MLS} \cite{hashimoto2025exploring}. Isso pode ser feito, por exemplo, por meio de uma troca de chaves \textit{Double Ratchet} pós-quântica para a criação de mensagens seguras em grupo. Essa abordagem permite reduzir a complexidade da troca de mensagens, ao mesmo tempo em que evita a exposição das chaves de todos os usuários caso apenas um deles seja comprometido.

Também são encontrados esforços para aplicar \gls{QKD} na comunicação por e-mail \cite{847_doberl2023quantum}, por exemplo, estabelecendo enlaces seguros baseados em \gls{QKD} entre servidores de e-mail, enquanto se utiliza \gls{PQC} na comunicação entre cliente e servidor.


\textbf{Camada de Rede.}
A camada de rede inclui endereçamento, roteamento e encaminhamento de pacotes. Um caso de uso relevante para \gls{PQC} e \gls{QKD} é a construção de \gls{VPN}s. As \gls{VPN}s funcionam por meio do encapsulamento de pacotes para criar conexões seguras na internet, protegendo o conteúdo da camada de rede, como endereços e a carga útil interna. Implementações populares, como \gls{IPsec} \cite{cano2024line, cano2024integrating}, WireGuard \cite{hulsing2021post} e OpenVPN, incorporam \gls{PQC} nos hosts de extremidade ou em dispositivos de rede, fornecendo criptografia na camada de rede. O uso de chaves geradas por \gls{QKD} para túneis seguros também tem sido explorado na literatura \cite{gao2025ipseq}, aprimorando os processos de autenticação e criptografia.

\textbf{Camada de Enlace.}
Para garantir criptografia ponto a ponto na camada de enlace, protocolos como o \gls{MACsec} estão sendo considerados para integração com \gls{PQC}. Enquanto versões anteriores do MACsec dependiam de chaves pré-compartilhadas em vez de mecanismos de encapsulamento de chaves, abordagens modernas exploram o uso de \gls{PQC} para autenticação e de \gls{QKD} para distribuição de chaves. Especificamente, o uso de \gls{PQC} para fornecer autenticação no acordo de chaves \gls{MKA} é proposto em \cite{buruaga2025versatile}. Além disso, o uso exclusivo de \gls{QKD} também vem sendo investigado. Esforços para estabelecer sessões \gls{MACsec} entre \textit{switches} utilizando chaves compartilhadas por meio de \gls{QKD} são documentados em trabalhos experimentais \cite{alia2025quantum}. O \gls{QKD} também vem sendo investigado para sistemas industriais e redes elétricas inteligentes \cite{alshowkan2022authentication}, particularmente para aplicações baseadas em SCADA.

==> tex/introduction.tex <==
\chapter{Introdução}
\label{chapter:introduction}

% ---------------------------------------------------------------------------
% Tutorial: Como estruturar o relatório e usar o template QuIIN (quiin.cls)
% ---------------------------------------------------------------------------

% Nesse primeiro parágrafo dá para detalhar melhor o que são cada um desses requisitos
A criptografia é necessária quando a comunicação ocorre por meio de um canal não confiável. Entre seus requisitos essenciais estão a autenticação, a confidencialidade, a integridade e o não repúdio. A autenticação é o processo de comprovar a identidade de uma parte. A confidencialidade garante que somente o destinatário pretendido tem acesso ao conteúdo da mensagem. A integridade assegura que o destinatário receba a mensagem original, sem quaisquer alterações. O princípio do não repúdio garante que o remetente realmente enviou a mensagem~\cite{khalifa}.

Há dois tipos de segurança criptográfica: a prática e a teórica ou incondicional. A segurança incondicional significa que o sistema é seguro, independentemente de o atacante possuir poder computacional ilimitado. A segurança prática leva em consideração a capacidade computacional limitada do atacante~\cite{massey}. Uma técnica criptográfica incondicionalmente segura é a \gls{OTP}, introduzida por Claude Shannon, que é capaz de criptografar a mensagem original por meio de uma operação de XOR bit a bit com a chave~\cite{shannon}. A \gls{OTP} é incondicionalmente segura, pois não há meios pelos quais o espião consiga extrair qualquer informação da mensagem cifrada~\cite{matt}~\cite{lucamarini}.

Os algoritmos de chave pública atualmente utilizados baseiam-se em problemas de fatoração de números inteiros e em logaritmos discretos, como o RSA e o ECC. Estes algoritmos são seguros na prática, pois consideram a complexidade computacional associada aos problemas de fatoração. Porém, o paradigma da computação quântica otimiza o tempo de processamento desses problemas de fatoração, tornando-os resolvíveis em tempo hábil. Esta característica permite inferir que computadores quânticos serão capazes de quebrar criptografias de chaves públicas~\cite{bhatia}. Por isso, novos algoritmos resistentes a ataques quânticos já estão sendo propostos. Uma abordagem utilizada por atacantes \cite{moral2024cybersecurity} é colher agora e descriptografar depois, ou seja, coletar dados ou chaves que são trafegados, utilizando algoritmos que não são resistentes a ataques quânticos, para que, quando surja um computador quântico, essas mensagens possam ser lidas. Em vista disso, é necessário garantir que as mensagens, ou ao menos as chaves de criptografia, não estejam sendo interceptadas.

Entre as formas utilizadas para garantir a idoneidade das chaves de criptografia estão as relacionadas às propriedades da mecânica quântica. A \gls{QKD} permite que chaves secretas sejam estabelecidas em duas pontas e garante que os parâmetros utilizados na geração dessas chaves não sejam capturados por um atacante~\cite{cao}. A \gls{QKD} é uma abordagem alternativa aos métodos convencionais de estabelecimento de chaves criptográficas, inicialmente fundamentada nos trabalhos de Wiesner~\cite{wiesner}, Bennet e Brassard~\cite{bennett} e Ekert~\cite{ekert}, e depende do envio e da detecção de sinais quânticos e de dados sobre medições e configurações para destilar uma chave segura.


A \gls{QKD} oferece segurança incondicional no processo de distribuição de chaves criptográficas. Quando essas chaves são empregadas em esquemas de cifragem como o One-Time Pad (OTP), é possível obter segurança teórica da comunicação. Contudo, essa abordagem exige a geração de chaves em volume equivalente ao tamanho dos dados transmitidos. Atualmente, o fluxo de geração de chaves para sistemas \gls{QKD} é limitado~\cite{zhang}. Os trabalhos de \cite{alia} e \cite{tang} são exemplos de abordagens para melhorar a distância alcançada na transmissão quântica de chaves e o fluxo de geração de chaves. A \gls{QKD} pode ser utilizada com outras técnicas de criptografia; se usada com cifras de bloco (e.g., \gls{AES}), esse protocolo já não será incondicionalmente seguro, mas será resistente a ataques por computadores quânticos~\cite{lucamarini}.

O \gls{ETSI} define padrões de interface entre aplicações seguras e a camada de gerenciamento de chaves da \gls{QKD}. O documento ETSI GS QKD 004~\cite{etsiqkd004} define uma interface que permite às aplicações consumir as chaves, estabelecendo uma comunicação entre duas extremidades. Há ainda o documento ETSI GS QKD 014~\cite{etsiqkd014}, que define uma API REST para solicitação de chaves por meio de requisições individuais, sem a necessidade de abrir a transmissão; além disso, essa definição não possui o conceito de sessões presente no ETSI GS QKD 004.

Um estudo aprofundado é necessário para planejar e viabilizar a integração das aplicações, protocolos e equipamentos clássicos com os equipamentos quânticos por meio do uso de padrões estabelecidos por fabricantes e/ou organizações de padronização, com o intuito de atender às crescentes demandas por comunicação segura em tempo real, resistente a computadores quânticos. O estudo deve identificar os desafios relacionados à implementação dos padrões de comunicação pelos fabricantes, ajustar, conforme forem necessárias, as aplicações para que consumam a partir dos equipamentos \gls{QKD} nos padrões especificados, observar limitações no fluxo de chaves e identificar alternativas que permitam manter um fluxo de dados viável na rede. 

A integração de redes clássicas com sistemas \gls{QKD} é primordial para o seu uso efetivo. Essa integração é capaz de beneficiar os setores da indústria que realizam trocas de informações muito sensíveis, como o financeiro, governamental, de defesa, de saúde, de petróleo e gás, entre outros. A adoção desse novo modelo de comunicação pode oferecer uma infraestrutura mais robusta e resistente a ataques futuros, fortalecendo a confiança digital em ambientes críticos.

A utilização de sistemas \gls{QKD} para distribuição de chaves inicia um novo paradigma na comunicação confiável. É necessário que a forma como os consumidores usam essas chaves seja alterada. A infraestrutura de chaves públicas é amplamente utilizada para trocar uma chave simétrica, mas deve ceder espaço à distribuição por meio de sistemas \gls{QKD}, capazes de trocar a chave simétrica, garantindo segurança por meio das propriedades da mecânica quântica. É necessário observar como as aplicações e protocolos disponíveis consomem chaves de criptografia atualmente e modelar casos de uso dessas aplicações utilizando esse novo paradigma de distribuição de chaves. Inicialmente, a infraestrutura de chave pública pode ser substituída por métodos de distribuição de chaves mais semelhantes ao utilizado pelo \gls{QKD}, como a chave pré-compartilhada, uma vez que a chave estará disponível em ambos os lados no sistema \gls{QKD}; porém, posteriormente, é necessário que o esquema de distribuição siga os padrões de comunicação especificados. 

A utilização de chaves provenientes de equipamentos \gls{QKD} também depende de novas técnicas de armazenamento e distribuição de chaves, uma vez que o fluxo de geração de chaves geradas pelos equipamentos \gls{QKD} é atualmente limitado. Melhorar a eficiência do fluxo de chaves é essencial para a garantia de um sistema teoricamente seguro; a persistência dessa limitação acarreta a necessidade de estudar e utilizar alternativas que sejam suficientemente seguras.

